Deep Learning for Visual Tracking: A Comprehensive Survey

Visual target tracking is one of the most sought-after yet challenging research topics in computer vision. Given the ill-posed nature of the problem and its popularity in a broad range of real-world scenarios, a number of large-scale benchmark datasets have been established, on which considerable methods have been developed and demonstrated with significant progress in recent years -- predominantly by recent deep learning (DL)-based methods. This survey aims to systematically investigate the current DL-based visual tracking methods, benchmark datasets, and evaluation metrics. It also extensively evaluates and analyzes the leading visual tracking methods. First, the fundamental characteristics, primary motivations, and contributions of DL-based methods are summarized from nine key aspects of: network architecture, network exploitation, network training for visual tracking, network objective, network output, exploitation of correlation filter advantages, aerial-view tracking, long-term tracking, and online tracking. Second, popular visual tracking benchmarks and their respective properties are compared, and their evaluation metrics are summarized. Third, the state-of-the-art DL-based methods are comprehensively examined on a set of well-established benchmarks of OTB2013, OTB2015, VOT2018, LaSOT, UAV123, UAVDT, and VisDrone2019. Finally, by conducting critical analyses of these state-of-the-art trackers quantitatively and qualitatively, their pros and cons under various common scenarios are investigated. It may serve as a gentle use guide for practitioners to weigh when and under what conditions to choose which method(s). It also facilitates a discussion on ongoing issues and sheds light on promising research directions.

==> Fig5.tex <==
\begin{figure*}[hbt!]
 \justify
\begin{subfigure}[b]{0.45\textwidth}
 \includegraphics[width=9cm, height=5cm]{Fig5-1.pdf}
\end{subfigure}%
\hspace{8mm}
\begin{subfigure}[b]{0.45\textwidth}
 \includegraphics[width=9cm, height=5cm]{Fig5-4.pdf}
\end{subfigure}
 \vspace{0mm}
 \justify
\begin{subfigure}[b]{0.45\textwidth}
 \includegraphics[width=9cm, height=5cm]{Fig5-2.pdf}
\end{subfigure}%
\hspace{8mm}
\begin{subfigure}[b]{0.45\textwidth}
 \includegraphics[width=9cm, height=5cm]{Fig5-3.pdf}
\end{subfigure}
 \caption{Performance comparison of visual tracking methods on VOT2018 dataset.}
 \label{fig:Results_VOT} 
 \vspace{-4mm}
\end{figure*}

==> Fig6-1.tex <==
\begin{figure*}[hbt!]
\centering
\vspace{-2mm}
\includegraphics[width=18cm, height=7cm]{Fig6.pdf}
\vspace{-4mm}
 \caption{Performance comparison of state-of-the-art visual tracking methods in terms of the most challenging attributes of the OTB2015 and LaSOT datasets.}
 \label{fig:AttResults_OTB_LaSOT} 
\vspace{-2ex}
\end{figure*}

==> Fig6.tex <==
\begin{figure*}[hbt!]
\justify
 \begin{subfigure}[b]{0.32\textwidth}
 \includegraphics[width=6cm, height=4cm]{Fig6-1.pdf}
 \end{subfigure}%
 \hspace{1mm}
 \begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=6cm, height=4cm]{Fig6-2.pdf}
 \end{subfigure}
 \hspace{1mm}
 \begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=6cm, height=4cm]{Fig6-3.pdf}
 \end{subfigure}%
  \vspace{-1ex}
  \justify
 \begin{subfigure}[b]{0.32\textwidth}
 \includegraphics[width=6cm, height=4cm]{Fig6-4.pdf}
 \end{subfigure}%
  \hspace{1mm}
 \begin{subfigure}[b]{0.32\textwidth}
 \includegraphics[width=6cm, height=4cm]{Fig6-5.pdf}
 \end{subfigure}
  \hspace{1mm}
 \begin{subfigure}[b]{0.32\textwidth}
 \includegraphics[width=6cm, height=4cm]{Fig6-6.pdf}
 \end{subfigure}
 \caption{Performance comparison of state-of-the-art visual tracking methods in terms of the most challenging attributes of the OTB2015 dataset.}
 \label{fig:AttResults_OTB} 
  \vspace{-4mm}
\end{figure*}

==> Fig7.tex <==
\begin{figure*}[hbt!]
\justify
 \begin{subfigure}[b]{0.32\textwidth}
 \includegraphics[width=6cm, height=4cm]{Fig7-1.pdf}
 \end{subfigure}%
  \hspace{1mm}
 \begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=6cm, height=4cm]{Fig7-2.pdf}
 \end{subfigure}
  \hspace{1mm}
 \begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=6cm, height=4cm]{Fig7-3.pdf}
 \end{subfigure}%
  \vspace{-1ex}
 \justify
 \begin{subfigure}[b]{0.32\textwidth}
 \includegraphics[width=6cm, height=4cm]{Fig7-4.pdf}
 \end{subfigure}%
  \hspace{1mm}
 \begin{subfigure}[b]{0.32\textwidth}
 \includegraphics[width=6cm, height=4cm]{Fig7-5.pdf}
 \end{subfigure}
  \hspace{1mm}
 \begin{subfigure}[b]{0.32\textwidth}
 \includegraphics[width=6cm, height=4cm]{Fig7-6.pdf}
 \end{subfigure}
 \caption{Performance comparison of state-of-the-art visual tracking methods in terms of the most challenging attributes of the LaSOT dataset.}
 \label{fig:AttResults_LaSOT} 
 \vspace{-4mm}
\end{figure*}

==> Table7.tex <==
\begin{table*}
\caption{Performance overview of visual tracking methods on VOT2018 dataset.} % title of Table
\centering % used for centering table
 \vspace{-2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{c c c c c c c c c c} % centered columns (4 columns)
\hline \hline 
\multirow{3}{*}{Visual Tracking Methods} & \multicolumn{5}{c}{Baseline} & \multicolumn{3}{c}{Unsupervised} & \multicolumn{1}{c}{Real-time} \\\cline{2-10}
& \multicolumn{1}{c}{EAO} & \multicolumn{2}{c}{A-R rank} & \multicolumn{2}{c}{Speed} & \multicolumn{1}{c}{Overlap} & \multicolumn{2}{c}{Speed} & \multicolumn{1}{c}{EAO}\\\cline{2-10}
& EAO & Overlap & Failures & Normalized & FPS & AUC & Normalized & FPS & EAO \\ \hline\hline
ECO \cite{ECO} & 0.2809 & 0.4762 & 17.6628 & 0.8031 & 3.7056 & 0.4025 & 0.9916 & 4.5321 & 0.0776 \\ \hline 
MCPF \cite{MCPF} & 0.2477 & 0.5042 & 25.9600 & 0.0779 & 0.4195 & \textbf{0.4440} & 0.0821 & 0.4273 & 0.0598 \\ \hline 
DCFNet \cite{DCFNet} & 0.1827 & 0.4646 & 35.2015 & \textbf{5.8744} & 27.2624 & 0.3269 & \textbf{7.3045} & 33.2206 & 0.1803 \\ \hline 
UPDT \cite{UPDT} & \textbf{0.3785} & 0.5302 & \textbf{10.4823} & 0.0810 & 0.4346 & \textbf{0.4546} & 0.0884 & 0.4697 & 0.0676 \\ \hline 
DaSiamRPN \cite{DaSiamRPN} & 0.3274 & \textbf{0.5673} & 21.4199 & - & - & - & - & - & - \\ \hline 
TRACA \cite{TRACA} & 0.1385 & 0.4306 & 53.6777 & 1.8143 & 10.0635 & 0.2587 & 3.4281 & 18.6393 & 0.1382 \\ \hline 
DeepSTRCF \cite{STRCF} & 0.3451 & 0.5165 & 13.1103 & 0.5193 & 2.9157 & 0.4365 & 0.5605 & 3.1144 & 0.0629 \\ \hline 
SiamRPN \cite{SiamRPN} & 0.2453 & 0.4910 & 28.6648 & \textbf{19.2695} & \textbf{104.4643} & 0.3586 & \textbf{19.5166} & \textbf{103.0445} & 0.2453 \\ \hline 
SA-Siam \cite{SA-Siam} & 0.2374 & 0.4999 & 27.8227 & - & 22.6941 & 0.4071 & - & 36.1594 & 0.2373 \\ \hline 
LSART \cite{LSART} & 0.3247 & 0.4919 & \textbf{12.7929} & 0.2967 & 1.7182 & 0.4389 & 0.2306 & 1.3242 & 0.0548 \\ \hline 
DRT \cite{DRT} & 0.3550 & 0.5076 & \textbf{12.7941} & 0.1175 & 0.4378 & 0.4240 & 0.1237 & 0.4568 & 0.0620 \\ \hline 
DAT \cite{DAT} & 0.1443 & 0.4310 & 42.0946 & \textbf{6.4338} & 28.6446 & 0.2871 & \textbf{8.5054} & \textbf{36.8791} & 0.1390 \\ \hline 
SiamMask \cite{SiamMask} & \textbf{0.3839} & \textbf{0.6040} & 16.2519 & - & - & - & - & - & - \\ \hline 
SiamRPN++ \cite{SiamRPN++} & \textbf{0.4169} & \textbf{0.5964} & 14.8653 & - & \textbf{34.3602} & \textbf{0.5015} & - & \textbf{37.0633} & \textbf{0.4169} \\ \hline 
  \end{tabular}
  \label{tab7}
 }
\vspace{-6mm}
\end{table*}
